VFSIE -- Development and Testing Framework for Federated Science Instruments

Recent developments in softwarization of networked infrastructures combined with containerization of computing workflows promise unprecedented compute anywhere and everywhere capabilities for federations of edge and remote computing systems and science instruments. The development and testing of software stacks that implement these capabilities over physical production federations, however, is not very practical nor cost-effective. In response, we develop a digital twin of the physical infrastructure, called the Virtual Federated Science Instrument Environment (VFSIE). This framework emulates the federation using containers and hosts connected over an emulated network, and supports the development and testing of federation stacks and workflows. We illustrate its use in a case study involving Jupiter Notebook computations and instrument control.

==> frontmatter.tex <==
% Volume frontmatter for NetSys 2021
% =====================================
\volume{XXX}{2020} % Volume number and year
\volumetitle{% Title of the volume (optional)
International Conference on Networked Systems 2021\\
(NetSys 2021)}
\volumeshort{% Short title of the volume (optional)
NetSys 2021}
\guesteds{% Multiple guest editors
Andreas Blenk, Mathias Fischer, Stefan Fischer, Horst Hellbrück, Oliver Hohlfeld, Andreas Kassler, Koojana Kuladinithi, Winfried Lamersdorf, Olaf Landsiedel, Andreas Timm-Giel, Alexey Vinel}

